Learning a Unified Embedding for Visual Search at Pinterest

At Pinterest, we utilize image embeddings throughout our search and recommendation systems to help our users navigate through visual content by powering experiences like browsing of related content and searching for exact products for shopping. In this work we describe a multi-task deep metric learning system to learn a single unified image embedding which can be used to power our multiple visual search products. The solution we present not only allows us to train for multiple application objectives in a single deep neural network architecture, but takes advantage of correlated information in the combination of all training data from each application to generate a unified embedding that outperforms all specialized embeddings previously deployed for each product. We discuss the challenges of handling images from different domains such as camera photos, high quality web images, and clean product catalog images. We also detail how to jointly train for multiple product objectives and how to leverage both engagement data and human labeled data. In addition, our trained embeddings can also be binarized for efficient storage and retrieval without compromising precision and recall. Through comprehensive evaluations on offline metrics, user studies, and online A/B experiments, we demonstrate that our proposed unified embedding improves both relevance and engagement of our visual search products for both browsing and searching purposes when compared to existing specialized embeddings. Finally, the deployment of the unified embedding at Pinterest has drastically reduced the operation and engineering cost of maintaining multiple embeddings while improving quality.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> main_ablation_exps.tex <==
\subsection{Metric Learning Experiments}\label{exp:metric}

% \subsubsection{Stanford Product Dataset}
% In this section, we aim to study 1) the effect of embedding dimension on the metric learning and 2) how our proposed classification network described in sec.~\ref{subsec:metric_learning} compare against other metric learning approaches.

% We evaluate on the public Stanford Product dataset with the same evaluation protocol described in ~\cite{songCVPR16}. The quality of the retrieval is measured using standard Recall@k metric. Our results are compared with 6 deep metric learning approaches, including 2 state-of-the-art methods: Distanced-weighted sampling with Margin loss\cite{samplingmatters} and Proxy loss\cite{nofusslearning} as shown in table \ref{tab:metric_stanford}.

% For fair comparison based on the same experiment settings, we implement these 2 SOTA methods\footnote{Reproduction of \cite{samplingmatters} is based on the source code provided by the authors}. The base feature network is fixed to be ResNet50~\cite{kaiming16} pre-trained on ImageNet~\cite{imagenet_cvpr09}, the same as~\cite{samplingmatters}. The last fully-connected layer of the base network is modified according to the desired embedding dimension with randomly initialized weights. The inputs are resized to $256 \times 256$, and then randomly cropped to size $224 \times 224$ during training with horizontal mirroring for data augmentation.  We use SGD optimizer with learning rate $1e-2$ and momentum $0.9$, and train the network for 60 epochs\footnote{We do not use Adam as described in~\cite{samplingmatters} as we could not reproduce their results with the optimizer. At the time of writing, we did not find the Stanford Products experiment source code available in the open source codebase.  Fortunately, SGD with standard classification hyperparameters achieves better performance than previously reported which we use as a baseline.}. Our reproduced numbers are slightly different but on the same ballpark. Our proposed method is compared with these baselines in Table~\ref{tab:metric_stanford}.
% \begin{table}
% \begin{center
% \begin{tabular}{l c c c c}
% \hline
% & Dim & R@1 & R@10 & R@100  \\
% \hline\hline
% Triplet Semihard\cite{structclust}& 64f &  66.7 & 82.4 & 91.9 \\
% Lifted  Struct\cite{songCVPR16}& 512f & 62.5 & 80.8 & 91.9 \\
% Struct Clust\cite{structclust}& 512f &  67.0 & 83.7 & 93.2 \\
% Npairs\cite{npairNIPS2016} & 64f & 67.7 & 83.8 & 93.0 \\
% Margin\cite{samplingmatters} & 128f & 72.7 & 86.2 & 93.8 \\
% Proxy\cite{nofusslearning} & 64f & 73.7 & - & - \\
% \hline
% Our implementations \\
% \hline
% Margin\cite{samplingmatters} & 128f & 74.9 & 88.3 & 95.5\\
% Proxy\cite{nofusslearning} & 128f & 67.0 & 81.3 & 90.3\\
% Ours & 128f & 71.1 & 85.2 & 93.2\\
% Margin\cite{samplingmatters} & 2048f  &  75.6 & 88.9 & \textbf{95.5}\\
% Proxy\cite{nofusslearning} & 2048f & 73.9 & 87.4 & 94.4\\
% Ours & 2048f & 75.1 & 87.8 & 94.6\\
% Ours(GN+D) & 2048f & 75.3 & 88.6 & 95.3\\
% Ours(GN+D) & 2048b & \textbf{76.3} & \textbf{89.2} & \textbf{95.5} \\
% \hline
% \end{tabular}
% \end{center}
% \caption{Recall@k on Stanford Products dataset. We see that our high-dimensional binarized embeddings surpass previous state-of-the-art.}
% \label{tab:metric_stanford}
% \end{table}

\begin{table}
\begin{center}
\label{tab:exp_subsampling}
\begin{tabular}{l c c c c}
\hline
& Dim & R@1 & R@10 & R@100  \\
\hline\hline
Margin\cite{samplingmatters} & 128f & 72.7 & 86.2 & 93.8 \\
Proxy\cite{nofusslearning} & 64f & 73.7 & - & - \\
\hline
Our implementations \\
\hline
Ours(GN+D) & 2048b & \textbf{76.3} & \textbf{89.2} & \textbf{95.5} \\
(subsampled 50\%) & 2048b & 75.4 & 88.7 & 95.2\\
(subsampled 10\%) & 2048b & 72.4 & 85.8 & 93.2\\
\hline
\end{tabular}
\end{center}
\caption{Recall@k on Stanford Products dataset. The results show the effect of subsampling.}
\label{tab:sampling_stanford}
\end{table}

\subsubsection{Shopping Dataset}
In this section, we compare the best sampling-based approach and our proxy-based approach on our Shopping dataset (sec.\ref{data:shopping}) for Recall@1. The base feature network for this experiment is SE-ResNext101\cite{senet} with the \textit{GN+D} binarization module. 

\begin{table}
\begin{center}
\begin{tabular}{l c c}
\hline
& Dim & R@1  \\
\hline\hline
Margin & 128f & 36.6 \\
Margin (min\_sample=5) & 2048f & 36.2 \\
Margin & 2048f & 37.6 \\
Margin & 2048b & 40.6 \\
Ours(subsampled 5\%) & 2048f & 40.7 \\
Ours(subsampled 5\%) & 2048b & \textbf{41.6} \\

\hline
\end{tabular}
\end{center}
\caption{Recall@1 on Shopping datasets.}
\label{tab:exp_shopping}
\end{table}

\begin{figure}[!ht]
\begin{center}

    \includegraphics[width=1.0\linewidth]{assets/margin_2048b_stela_retrieval.png}
Margin loss\cite{samplingmatters} Results

    \includegraphics[width=1.0\linewidth]{assets/softmax_2048b_stela_retrieval.png}
Our Results
\end{center}
   \caption{Quantitative retrieval results. The queries are randomly sampled from test set. The retrieval results are ranked by increasing distance from left to right}
\label{fig:metric_qualitative}
\end{figure}

\subsection{Results}
As shown in table~\ref{tab:metric_stanford} and~\ref{tab:exp_shopping}, the best results are when we combine our classification metric learning approach on high-dimensional embeddings with our binarization module. 

We observe the common trend in all experiments: high-dimensional binary embeddings \textbf{improve}  results for all reproduced metric learning techniques. Our subsampled classification approach outperform sampling-based approach. From the qualitative results shown in figure \ref{fig:metric_qualitative}, our approach seems to exhibit stronger orientation invariance and sementic consistency.

It is interesting to note that when we filter our training dataset such that minimum samples per class is 5, the default setting from \cite{samplingmatters}, R@1 drops by 1.4 percentage point. We have the similar observation in our ablation experiments (table\ref{tab:ablation}). This finding contradicts the traditional wisdom for training classifier: metric learning benefits from having more classes, even when the number of samples are small.

 Binarizing the high dimensional embeddings not only save the memory footprint, but improve the image retrieval performance. Our method surpasses previous SOTA\cite{nofusslearning} R@1 by 3.4 percentage point with the same bytesize of the embeddings.

We also show the effect of subsamping (sec. \ref{tab:exp_subsampling}). When using only 50\% of all classes used for each batch, our method achieves SOTA performance. The performance drops as less classes are used during each batch.


==> main_metric_learning.tex <==

\subsection{Web-scale Multi-task Metric Learning}
Being able to effectively do metric learning on web-scale data is important to deliver practical computer vision applications\cite{visualdiscoverypinterest}\cite{visualsearchbing}\cite{visualsearchebay}\cite{visualsearchalibaba}. As the web-scale datasets often contains millions of images and hundreds of thousands classes, sampling-based metric learning methods often struggles to select informative samples for model to train. In conjunction with optimizing for multiple objectives in different tasks, selecting informative samples within a mini batch becomes infeasible.

In this work, we use proxy-based metric learning method\cite{our_paper} to learn \textbf{high-dimensional binary} embeddings with softmax loss on the web-scale datasets. The training architecture is the standard \textbf{classification network without bias} and use the output of the last fully-connected layer as the embedding. Our choices eliminates the need to find meaningful negatives during training batch construction, and it is easy for us to perform multi-task learning. As suggested in \cite{our_paper}, we need subsampling to scale up proxy-based metric learning to web-scale datasets. In the following sections, we will detail the implementations of subsampling module and how we construct the model for multi-task metric learning.

\subsection{Subsampling Module}
\label{subsec:subsampling}
Fitting all proxies in memory during training may not be possible with high-dimensional embeddings and large number of classes. To address this issue, we implement the \textbf{subsampling module}. As shown in Figure\ref{fig:sampling},  for each training batch, the subsampling modules samples a subset of all classes for optimization. The sampled subset is guaranteed to have all the class labels in the training batch. The module also generates a new list of labels for the training batch in accordance with the position of the sampled class in the subset. This new list of labels will later be used for loss function. The pseudocode for the forward pass is provided at \ref{alg:subsampling}.



% Song et al\cite{songCVPR16} has done ablation studies on three public datasets and concluded that the dimension of the embeddings does not affect the performance.

\begin{algorithm}
\caption{Sub-sampling}\label{alg:subsampling}
\begin{flushleft}
\textbf{Input:} targets, num\_samples\\
\textbf{Output:} sampled\_labels, remapped\_targets\\ 
\end{flushleft}
\begin{algorithmic}[1]
\REQUIRE $len(targets) \leq num\_samples$
\STATE $sampled\_labels \leftarrow set(targets)$
\WHILE{$len(sampled\_labels) \leq num\_samples$} 
    
        \STATE{$s \leftarrow sample(all\_labels)$}
        \IF{$s \notin sample\_labels$} 
            \STATE {$sample\_labels.add(s)$}
        \ENDIF
\ENDWHILE

\STATE $sampled\_labels \leftarrow list(sampled\_labels)$
\STATE $remapped\_targets \leftarrow list([])$
\FORALL{$t \in targets$}
    \FORALL{$index, label \in enumerate(sampled\_labels)$}
        \IF{$t = label$} 
            \STATE {$remapped\_targets.add(index)$}
        \ENDIF
    \ENDFOR
\ENDFOR

\RETURN $sampled\_labels, remapped\_targets$
\end{algorithmic}
\end{algorithm}

==> main_multitask.tex <==
\subsection{Multi-Task}
\label{sec:multitask}

% In previous years at Pinterest, multiple specialized image embeddings were developed targeting three domains of focus for our company: organic, camera, and shopping. In 2015, we first launched Visual Search across our corpus of billions of images allowing users to visual search with any image in our corpus. In 2017, we launched Camera based Visual Search allowing users to search our corpus of images with their phone cameras. In the same year, we also launched Visual Shopping, allowing users to Shop similar looking products.

% With limited human resources, in 2018 we faced challenges of (1) \textit{Model Staleness}: Each specialized embedding requires its own maintainence and iterations for improvement. Given a near constant team size, growing the number of specialized embeddings is impractical (2) \textit{Dataset Underutilization}: Though each visual search product is biased towards different types of content, there are still overlaps in user behavior (e.g. User takes a picture of a product screenshot with their Camera phone). Ideally we want to return the best results to our users irregardless of the interface for querying. (3) \textit{Operational Cost}: Each specialized embedding results in a linear increase in feature extraction cost and serving requirements. 

\begin{figure}[t]
\begin{center}
\includegraphics[width=1.0\linewidth]{assets/training_datasets.png}
\end{center}
   \caption{Visualization of our multi-task training datasets}
\label{fig:training_datasets}
\end{figure}

With both business constraints and the interest of improved performance, we look to learn one image representation that can replace each specialized embedding. We first describe our training datasets (also visualized in ~\ref{fig:training_datasets} and then discuss more details into our multi-task architecture. 

\subsubsection{Related Images Dataset}
The Related Images dataset is generated through feedback from our users in a similar manner to the Memboost described in~\cite{relatedpins}. This allows us to generate image sets where a given query image has a set of related images ranked via engagement. We apply a set of strict heuristics (e.g. number of impressions and interactions for each image in the set) to reduce the label noise of the dataset, resulting in around 800K images in 15K image sets. 

\subsubsection{Shopping Dataset}
\label{data:shopping}
The Shopping dataset is a human labeled dataset containing 340K images with 189 product class label (e.g. Bar Stools) and 50K instance labels. Images with the same instance label are either exact matches are very visually similar.

\subsubsection{Camera Dataset}
The Camera dataset is a human labeled dataset containing 540K images with 2K semantic classes. These semantic classes range from broad categories (e.g. tofu) to fine-grained classes (e.g. the same denim jacket in camera and product shots). Most importantly, this dataset contains a mix of product, camera, and organic images under the same semantic label. query images biased towards Camera images. Query images for this dataset were generated with loose heuristics (e.g. certain phones generate images of the same size)

\subsubsection{Multi-Task Architecture}
As shown in Figure~\ref{fig:architecture}, for every mini-batch, we mix in uniformly each of the above datasets specializing in one of the three domains of focus. At Company X, the want the image representation to be multi-faceted so naturally we share common parameters up to the image embedding layer, followed by task-specific heads for different objectives. Every objective is unique to a specific dataset (no two datasets share the same objective) so for simplicity, we ignore the gradient contributions of images on tasks that it does not have data for. We present more details in specific architectural decisions regarding our multi-task model in the next Section.
